Unsupervised Recognition of Unknown Objects for Open-World Object Detection

Open-World Object Detection (OWOD) extends object detection problem to a realistic and dynamic scenario, where a detection model is required to be capable of detecting both known and unknown objects and incrementally learning newly introduced knowledge. Current OWOD models, such as ORE and OW-DETR, focus on pseudo-labeling regions with high objectness scores as unknowns, whose performance relies heavily on the supervision of known objects. While they can detect the unknowns that exhibit similar features to the known objects, they suffer from a severe label bias problem that they tend to detect all regions (including unknown object regions) that are dissimilar to the known objects as part of the background. To eliminate the label bias, this paper proposes a novel approach that learns an unsupervised discriminative model to recognize true unknown objects from raw pseudo labels generated by unsupervised region proposal methods. The resulting model can be further refined by a classification-free self-training method which iteratively extends pseudo unknown objects to the unlabeled regions. Experimental results show that our method 1) significantly outperforms the prior SOTA in detecting unknown objects while maintaining competitive performance of detecting known object classes on the MS COCO dataset, and 2) achieves better generalization ability on the LVIS and Objects365 datasets.

==> discussion.tex <==

\section{Discussions} \label{sec:discussion}


{\small\textbf{Differences from fixed-point quantization approaches.}}
Our GroupNet is different from fixed-point quantization approaches~\cite{zhang2018lq, zhuang2018towards, zhou2016dorefa, mishra2018apprentice} in both the quantization algorithm and its underlying inference implementation. 

Note that in conventional fixed-point methods, the inner product between fixed-point weights and activations can be computed by bitwise operations.
Let ${\bw} \in {\mathbb{R}^M}$ and $\ba \in {\mathbb{R}^M}$
be the weights and activations, respectively.  they can be encoded by a linear combination of binary bases, respectively. 
In particular, $\bw$ and $\ba$ can be encoded by ${\bf{b}}_i^w \in {\{ - 1,1\} ^M}$ and ${\bf{b}}_i^a \in {\{ - 1,1\} ^M}$, where $i = 1,...,P$, respectively. Let $Q_P(\cdot)$ be any quantization function, and for simplicity, we here consider uniform quantization only. Then, the inner product of $\bw$ and $\ba$ can be approximated by
\begin{equation} \label{eq:fixed-point}
{Q_P}({{\bf{w}}^\mathrm{T}}){Q_P}({\bf{a}}) = \sum\limits_{i = 0}^{P-1} {\sum\limits_{j = 0}^{P-1} {{2^{i + j}}} } ({\bf{b}}_i^w \xor {\bf{b}}_j^a).
\end{equation}
where $\xor$ indicates the binary inner product, which can be efficiently implemented by
$\rm popcount$ and $\rm xnor$ bit-wise instructions that are commonly equipped in modern computers. According to Eq. (\ref{eq:fixed-point}), the computational complexity is $O(MP^2)$ for the fixed-point inner product.
Bearing the group-wise binary decomposition in Section \ref{sec:decomposition} in mind, it can be easily realized that the proposed GroupNet with $K$ bases has the same computational complexity with the conventional $P$-bit fixed point quantization when $K = 2^P$. However, compared with the $P$-bit fixed point quantization, the proposed GroupNet with $2^P$ bases introduces extra additions from the fusion of decomposition branches. It is worth noting that the convolution is implemented with two steps: $\rm im2col$ and $\rm GEMM$. The high-precision additions can be efficiently merged into the $\rm im2col$ operation of the succeeding layer during implementation. For $\rm im2col$ operation, most of the time is spend on data rearrangement, an extra tensor addition will have a very limited influence on its execution time.
Moreover, the extra additions only account for a small portion of the overall network complexity, which intrinsically limits the impact on the overall speed.
To justify our analysis, we provide speedup evaluations in Section \ref{sec:speed_benchmarks}. We also provide the analysis of the runtime training and inference memory cost in Section \ref{exp:runtime_memory}.


To emphasize, 
the proposed GroupNet enables much more flexible design of the quantization algorithm. 
Benefiting from the group-wise binary decomposition, the proposed GroupNet allows more fine-grained exploration space, where the quantization levels can be chosen from the continuous positive integer domain. In contrast, conventional fixed-point quantization requires the quantization levels to be the power of 2. For example, the bit-width of GroupNet with 5 bases is between 2-bit and 3-bit. Thus, GroupNet enjoys a flexible trade-off between complexity and accuracy by setting appropriate $K$.
Moreover, as introduced in Section \ref{sec:segmentation} and Section \ref{sec:detection}, 
our GroupNet is demonstrated to be more efficient in exploiting task-specific information or structures to compensate the quantization information loss.

Moreover, we define the model size of the full-precision model as $\Omega$. Then, the model size for GroupNet with $K$ bases becomes $K\Omega/32$ and the one for $P$-bit fixed-point quantization is $P\Omega/32$.

Based on the above analysis, we summarize that the proposed GroupNet
introduces small additional run-time cost caused by the extra addition operations, however, provides benefits in algorithm flexibility and performance.


\noindent\textbf{\kui{Differences between GroupNet
and 
other multiple binarizations methods.}}
In \cite{lin2017towards}, a linear combination of binary weight/activations bases are obtained from the full-precision weights or activations without being directly learned. In contrast, we directly design the binary network structure, where binary weights are end-to-end optimized. ~\cite{fromm2018heterogeneous, tang2017train, guo2017network, li2017performance} propose to recursively approximate the residual error and obtain a series of binary maps corresponding to different quantization scales.
However, it is a sequential process which cannot be paralleled. Also, all previous multiple binarizations methods belong to local tensor approximation. 
In contrast to value approximation, we propose a group decomposition approach to approximate the full-precision network. Moreover, tensor-based methods are tightly designed to local value approximation and may be hardly generalized to other tasks accordingly. In addition, our group decomposition strategy achieves much better performance than tensor-level approximation as shown in Section~\ref{sec:group_space}.

   
